Theory Support for the Excited Baryon Program at the Jlab 12 GeV Upgrade

This document outlines major directions in theoretical support for the measurement of nucleon resonance transition form factors at the JLab 12 GeV upgrade with the CLAS12 detector. Using single and double meson production, prominent resonances in the mass range up to 2 GeV will be studied in the range of photon virtuality $Q^2$ up to 12 GeV$^2$ where quark degrees of freedom are expected to dominate. High level theoretical analysis of these data will open up opportunities to understand how the interactions of dressed quarks create the ground and excited nucleon states and how these interactions emerge from QCD. The paper reviews the current status and the prospects of QCD based model approaches that relate phenomenological information on transition form factors to the non-perturbative strong interaction mechanisms, that are responsible for resonance formation.

==> EBAC/status_ebac.tex <==

%\documentclass[preprint,aps,tightenlines,showpacs,superscriptaddress]{revtex4}
%\documentclass[prl,eqsecnum,twocolumn,floats,aps,showpacs,superscriptaddress]{revtex4}
%\usepackage[dvips]{graphicx}
%\usepackage{dcolumn}
%\usepackage{bm}
%\usepackage{epsfig}

%\usepackage{showlabels}
%\renewcommand{\case}{\frac}




%\section [Research Program at Excited Baryon Analysis Center}
%\\
\begin{centering}
{T.-S. Harry Lee for the EBAC collaboration}
\end{centering}

\vspace{0.1in}
\begin{center}
{\bf EBAC Strategy}
\end{center}
\vspace{0.1in}


The objective of EBAC is more than just the usual
partial-wave analysis. We  not only want to
 extract the $N^*$ parameters from
the world data of meson production reactions, but also
to map out the
quark-gluon substructure of $N^*$ states. This
requires a full dynamical coupled-channels 
analysis~\cite{Lee06} which accounts for both 
the unitarity conditions and the reaction mechanisms from short to large distances.
The channels included in the analysis
are two-particles $\gamma^* N, \pi N, \eta N, 
K\Lambda, K\Sigma, \omega N$ states and the crucial three-particle
$\pi\pi N$ state which includes $\pi\Delta, \rho N, \sigma N$ resonant components.
The resonance parameters are extracted
from the poles on the unphysical sheets of the complex-energy plane, 
which can be more
directly compared with the pedictions from hadron models and LQCD.
Fig.~\ref{fig:ebac-plan} illustrates the EBAC strategy.

\vspace{0.1in}
\begin{center}
{\bf Status of EBAC Analysis}
\end{center}
\vspace{0.1in}

The analysis of $\pi N, \gamma^*N \rightarrow \pi N, \eta N, \pi\pi N$ has 
been performed~\cite{jlms,jlmss,djlss,kjlms}. The resonance parameters of
the low-lying  $N^*$ states
with masses below about 1.7 GeV (red arrows in Fig.2) have been extracted.
 The higher mass $N^*$ states ( dashed arrows in Fig.2), 
suggested by the Particle Data Group, are still being investigated.
The main task is to include $K\Lambda$, $K\Sigma$, and $\omega N$ 
channels in the analysis. Furthermore an effort has been devoted to
recover the old data of $\pi N \rightarrow \pi\pi N$ reactions which
are essential in pinning down the higher mass $N^*$ states. New data from
new hadron facilities, such as JPARC in Japan,  may be essential
 in making  conclusive determinations of some of these "elusive" $N^*$ states.

With the data from 12 GeV upgrade, the EBAC analysis needs to be extended
to account for reaction mechanisms at high momentum transfer.
It is necessary to describe the non-resnant mechanisms directly in terms
of quark-gluon degrees of freedom. The results from the DSE approach,
described in another contribution to these proceedings, will be useful 
to make progress in this direction.


\begin{figure}[h]
\centering
\includegraphics[clip,width=14cm]{STATUS_EBAC/ebac-plan.eps}
\caption{EBAC Strategy}
\label{fig:ebac-plan}
\end{figure}
\newpage

\begin{figure}[h]
\centering
\includegraphics[clip,width=14cm]{STATUS_EBAC/ebac-status.eps}
\caption{Status of $N^*$ study at EBAC}
\label{fig:ebac-status}
\end{figure}

\clearpage
%References
\begin{thebibliography}{99}

\bibitem{jlms}
B. Julia-Diaz, T.-S.H. Lee, A. Matsuyama, T. Sato,
Phys.Rev. {\bf C76}, 5201 (2007)

%
\bibitem{jlmss}
B. Julia-Diaz, T.-S.H. Lee, A. Matsuyama, T. Sato, L.C. Smith
   ,Phys.Rev.C77:045205,2008
\bibitem{djlss}
  J. Durand, B. Julia-Diaz, T.-S.H. Lee, B. Saghai, T. Sato,
   Phys.Rev.C78:025204,2008.

\bibitem{kjlms}
H. Kamano, B. Julia-Diaz, T.-S.H. Lee, A. Matsuyama, T. Sato
   submitted to Phys. Rev. C, e-Print: arXiv:0807.2273 [nucl-th]
\end{thebibliography}

%\end{document}


